A partition of unity approach to fluid mechanics and fluid-structure interaction

For problems involving large deformations of thin structures, simulating fluid-structure interaction (FSI) remains challenging largely due to the need to balance computational feasibility, efficiency, and solution accuracy. Overlapping domain techniques have been introduced as a way to combine the fluid-solid mesh conformity, seen in moving-mesh methods, without the need for mesh smoothing or re-meshing, which is a core characteristic of fixed mesh approaches. In this work, we introduce a novel overlapping domain method based on a partition of unity approach. Unified function spaces are defined as a weighted sum of fields given on two overlapping meshes. The method is shown to achieve optimal convergence rates and to be stable for steady-state Stokes, Navier-Stokes, and ALE Navier-Stokes problems. Finally, we present results for FSI in the case of a 2D mock aortic valve simulation. These initial results point to the potential applicability of the method to a wide range of FSI applications, enabling boundary layer refinement and large deformations without the need for re-meshing or user-defined stabilization.

==> input_files/classical_ALE.tex <==

\subsection{Classical FEM approach to the ALE Navier-Stokes  problem}
\begin{itemize}
	\item We now consider a time dependent physical domain $\Omega_f\subset\realset^d\times\left[0, T\right]$. At each time point $t\in[0,T]$, we define $\Omega_{f,t} := \Omega_f(\cdot,t)\in\realset^d$, as well as its boundary $\Gamma_t$.
	
	\item The incompressible Navier-Stokes equation in arbitrary Lagrangian-Eulerian (ALE) form can be written as follows: find $(\bv,p)$ such that
	\begin{subequations}
		\label{eq:ALE}
		\begin{align}
			\rho\partial_t \bv + \rho(\bv - \hat{\bv} )\cdot\nabla\bv - \divergence \bsigma& = \mathbf{0} && \text{ in } \Omega_f, \label{eq:ALE_con_mom} \\
			\divergence \bv & = 0 && \text{ in } \Omega_f, \\
			\bv & = \bv_D && \text{ on } \Gamma_f^D \\
			\bsigma \cdot \bn & = \bt_N &&  \text{ on } \Gamma^N_f, \\
			\bv(\cdot, 0)  & = \bv_0  && \text{ in } \Omega_{f,0}
			\end{align}
	\end{subequations}
	\item Here, $\partial_t$ is a time derivative with respected to a fixed point in a reference domain, $\Lambda_f$. 
	\item Let $\mathcal{P}:\Lambda_f\times[0,T]\rightarrow\Omega_f$ be an arbitrary mapping such that $\mathcal{P}\in C^1(\Lambda_f\times\left[0,T\right])$ and $\mathcal{P}(\cdot,t) = \mathcal{P}_t:\Lambda_f\rightarrow\Omega_{f,t}$ is a bijective mapping $\forall \hspace{1mm} t\in\left[0,T\right]$. Thus, for any coordinate $\bx\in\Omega_t$ there is a $\bX\in\Lambda_f$ such that $\bx = \mathcal{P}(\bX,t)$.
	\item Now, the relation between the ALE time derivative and Eulerian one can be expressed using the chain rule:
	\begin{align}
		\partial_t f = \left.\frac{\partial f}{\partial t}\right|_{\bx} + \frac{\partial \mathcal{P}(\bX,t)}{\partial t} \cdot\left.\frac{\partial f}{\partial \bx}\right|_\bx = \left.\frac{\partial f}{\partial t}\right|_{\bx} + \hat{\bv} \cdot \nabla f
	\end{align}
	where $\hat{\bv}$ is the arbitrary grid velocity and $f$ is a given function.
	
	\item We approximate the ALE time derivative using the implicit BDF(2) thus we converting Equation~\ref{eq:ALE_con_mom} into:
	\begin{equation}
		\rho\frac{3\bv_n - 4\bv_{n-1} + \bv_{n-2}}{2\Delta t} + \rho(\bv_n - \hat{\bv}_n) \cdot\nabla\bv_n - \nabla\bsigma(\bv_n,p_n) = \mathbf{0}
	\end{equation}
	\item $(\bv_n,p_n)$ represents the current unknown field, while $\bv_{n-1}$ and $\bv_{n-2}$ are the velocity fields obtained at the previous two time points.
	\item $\Delta t$ represents the time step.
	\item $\hat{\bv}_n$ is a given grid velocity field
	\item Before writing the weak form of the problem, we define the following function spaces in the ALE coordinates:
	\begin{align*}
		\boldsymbol{\mathV}(t) &= \bH^1(\Omega_{f,t}), && \boldsymbol{\mathV}_D(t) = \{\bv\in\boldsymbol{\mathV} \defas \bv = \bv_D \text{ on } \Gamma_f^D  \} \\
		\mathW(t) &= L^2(\Omega_{f,t}), && \boldsymbol{\mathV}_0(t)  = \{\bv\in\boldsymbol{\mathV} \defas \bv = \mathbf{0} \text{ on } \Gamma_f^D \}
	\end{align*}
	
	\item For a given time step $n$, we can write the weak formulation of problem~\ref{eq:ALE} as: find $(\bv_n,p_n)\in\boldsymbol{\mathV}_D(t)\times\mathW(t)$ such that $\forall (\bw,q)\in\boldsymbol{\mathV}_0(t)\times \mathW(t)$ we have that
	\begin{align*}
		\int_{\Omega_{f,t}}\rho \bw \cdot \frac{3\bv_n-4\bv_{n-1}+\bv_{n-2}}{2\Delta t} + \rho\bw\cdot ((\bv_n - \hat{\bv}_n)\cdot\nabla\bv_n)  \hspace{1mm} d\Omega  & +  \\
		\int_{\Omega_{f,t}}\nabla\bw : \bsigma(\bv_n,p_n) \hspace{1mm} + q\divergence\bv_n \hspace{1mm} d\Omega &= 0
	\end{align*}
	
	\item For spatial discretization, we use P2-P1 Taylor-Hood elements, with a set-up similar to that of the Stokes problem.
	
	\item Due to the problem being non-linear, we use the iterative Newton-Raphson algorithm in order to approximation of the solution. Our convergence criterion is having the $L^2$ norm of the residual below the threshold value of $10^{-6}$ .
\end{itemize}
